Object Localization and Size Estimation from RGB-D Images

Depth sensing cameras (e.g., Kinect sensor, Tango phone) can acquire color and depth images that are registered to a common viewpoint. This opens the possibility of developing algorithms that exploit the advantages of both sensing modalities. Traditionally, cues from color images have been used for object localization (e.g., YOLO). However, the addition of a depth image can be further used to segment images that might otherwise have identical color information. Further, the depth image can be used for object size (height/width) estimation (in real-world measurements units, such as meters) as opposed to image based segmentation that would only support drawing bounding boxes around objects of interest. In this paper, we first collect color camera information along with depth information using a custom Android application on Tango Phab2 phone. Second, we perform timing and spatial alignment between the two data sources. Finally, we evaluate several ways of measuring the height of the object of interest within the captured images under a variety of settings.

==> eval.tex <==
\section{Evaluation}
\label{sec:eval}
In Figure~\ref{fig:human}, we show the result of our size estimation on people.
\begin{figure}[ht]
\centering
%\subfloat[{Actual: 167cm, Computed: 159cm, Error: 8cm}]{\includegraphics[width=\figurewidthG]{figures/person1.png}} \hspace{0.1in}
%\subfloat[{Actual: 92cm, Computed: 86cm, Error: 6cm}]{\includegraphics[width=\figurewidthG]{figures/person2.png}} %\hspace{0.1in}
\subfloat{\includegraphics[width=\figurewidthG]{person1.png}} \hspace{0.1in}
\subfloat{\includegraphics[width=\figurewidthG]{person2.png}} %\hspace{0.1in}
\vspace*{-0.1in}
\caption{Evaluation on people.}
\vspace*{-0.1in}
\label{fig:human}
\end{figure}


In Figure~\ref{fig:boxes}, we show the result of our size estimation on packing boxes
arranged in different configurations.
\begin{figure}[ht]
\centering
%\subfloat[{Actual: 109cm, Computed: 113cm, Error: 4cm}]{\includegraphics[width=\figurewidthG]{figures/box1.png}} \hspace{0.1in}
%\subfloat[{Actual: 92cm, Computed: 86cm, Error: 6cm}]{\includegraphics[width=\figurewidthG]{figures/box2.png}} %\hspace{0.1in}
\subfloat{\includegraphics[width=\figurewidthG]{box1.png}} \hspace{0.1in}
\subfloat{\includegraphics[width=\figurewidthG]{box2.png}} %\hspace{0.1in}
\vspace*{-0.1in}
\caption{Evaluation on different configuration of boxes.}
\vspace*{-0.1in}
\label{fig:boxes}
\end{figure}

In Figure~\ref{fig:objects}, we show the result of our size estimation on other different
objects.
\begin{figure}[ht]
\centering
%\subfloat[{Actual: 38cm, Computed: 35cm, Error: 3cm}]{\includegraphics[width=\figurewidthG]{figures/object1.png}} \hspace{0.1in}
%\subfloat[{Actual: 34cm, Computed: 37cm, Error: 3cm}]{\includegraphics[width=\figurewidthG]{figures/object2.png}} %\hspace{0.1in}
\subfloat{\includegraphics[width=\figurewidthG]{object1.png}} \hspace{0.1in}
\subfloat{\includegraphics[width=\figurewidthG]{object2.png}} %\hspace{0.1in}
\vspace*{-0.1in}
\caption{Evaluation on different objects.}
\vspace*{-0.1in}
\label{fig:objects}
\end{figure}

As we see our methods can estimate dimenions of objects very accurately when point cloud
information is available and is able to clearly segment out the object to be measured.

